Sequential Sampling Equilibrium

This paper introduces an equilibrium framework based on sequential sampling in which players face strategic uncertainty over their opponents' behavior and acquire informative signals to resolve it. Sequential sampling equilibrium delivers a disciplined model featuring an endogenous distribution of choices, beliefs, and decision times, that not only rationalizes well-known deviations from Nash equilibrium, but also makes novel predictions supported by existing data. It grounds a relationship between empirical learning and strategic sophistication, and generates stochastic choice through randomness inherent to sampling, without relying on indifference or choice mistakes. Further, it provides a rationale for Nash equilibrium when sampling costs vanish.

==> Tables/table-payoffs-actions-alldata.tex <==
\begin{tabular}{l@{\extracolsep{4pt}}cccc@{}}
\hline\hline
&\multicolumn{2}{c}{$\{$Player $M$ chooses $a$$\}$}  &  \multicolumn{2}{c}{$\{$Player $C$ chooses $a$$\}$} \\
\cline{2-3} \cline{4-5}
               &           OLS &          Logit &            OLS &          Logit \\
& (1) & (2) & (3) & (4) \\
\hline
    $\delta_M$ &         0.015 &          0.061 & -0.854$^{***}$ & -3.910$^{***}$ \\
               &       (0.030) &        (0.121) &        (0.025) &        (0.148) \\ [.25em]
     Intercept & 0.451$^{***}$ & -0.198$^{***}$ &  0.889$^{***}$ &  1.790$^{***}$ \\
               &       (0.014) &        (0.055) &        (0.011) &        (0.069) \\

\hline
(Pseudo) R$^2$ &          0.00 &           0.00 &           0.24 &           0.19 \\
  Observations &        3402 &           3402 &         3486 &           3486 \\
\hline\hline
\multicolumn{4}{l}{\footnotesize Heteroskedasticity-robust standard errors in parentheses. }\\
\multicolumn{4}{l}{\footnotesize $^{*}$ \(p<0.1\), $^{**}$ \(p<0.05\), $^{***}$ \(p<0.01\).}\\
\end{tabular}
